Planning Human-Robot Co-manipulation with Human Motor Control Objectives and Multi-component Reaching Strategies

For successful goal-directed human-robot interaction, the robot should adapt to the intentions and actions of the collaborating human. This can be supported by musculoskeletal or data-driven human models, where the former are limited to lower-level functioning such as ergonomics, and the latter have limited generalizability or data efficiency. What is missing, is the inclusion of human motor control models that can provide generalizable human behavior estimates and integrate into robot planning methods. We use well-studied models from human motor control based on the speed-accuracy and cost-benefit trade-offs to plan collaborative robot motions. In these models, the human trajectory minimizes an objective function, a formulation we adapt to numerical trajectory optimization. This can then be extended with constraints and new variables to realize collaborative motion planning and goal estimation. We deploy this model, as well as a multi-component movement strategy, in physical collaboration with uncertain goal-reaching and synchronized motion tasks, showing the ability of the approach to produce human-like trajectories over a range of conditions.

==> archive/scraps.tex <==

% synchronisation task: human and robot are controlling different axes where human movements determine the phase of the robot movements, we do not need to have a strategy switch on the robot as the human drives the phase anyway and would make the switch by themselves
% role transition: robot moves towards estimated goal position, drops impedance at the transition point so that the human does the fine positioning. Can benchmark against full robot trajectory, human alone (?), or standard impedance control w/ linear trajectory

% tasks (goal-oriented): shelf assembly (difference in robot goal knowledge)


% EXP1 shelf assembly (co-manipulation)
% - EXP1a: the robot knows the goal in the z-axis and we show synchronization
% - EXP2a: the robot does not know the goal in the z-axis and we show the switch by reducing gravity compensation

% EXP2 circuit board assembly (hand-over): we show that the switch determines the handover point
% - The robot picks up a component from far away, showing that the human can easily intervene after the switch
% - Test from multiple starting points and goal widths

\begin{eqnarray}
    x^h(t) & = & \mathtt{bell}(x^h_0, g) \\
    F^h(t) & = & \mathtt{hum\,imp}(x(t)-x^h(t))*(1+\epsilon) \\
    J^r(F_h) & = & \mathbb{E}_{s,F_h} \int_0^\infty \bigg( e^{-t/\gamma} R\left(s(t),g\right) - \nu \Vert F_h(t) \Vert^2 \bigg) dt \label{eq:human_obj}
\end{eqnarray}

\begin{table}
\begin{tabular}{ r | l | l }
 & Human & Robot \\ \hline
Error & $|x-g|<w$ & $E_g |x-g|<w$ \\
Effort & $|\tau|$ & $|K|$ \\
Noise & $\propto \tau$ & - \\
\end{tabular}
\end{table}
